A Focused Mapping Study on Customization in Interactive Technologies for Autism

Autism Spectrum Disorder (ASD) is neurodevelopmental condition characterized by social interaction and communication difficulties, along with narrow and repetitive interests. Being an spectrum disorder, ASD affects individuals with a large range of combinations of challenges along dimensions such intelligence, social skills, or sensory processing. Hence, any interactive technology for ASD ought to be customizable to fit the particular profile of each individual that uses it. The goal of this paper is to characterize the support of customization in this area. To do so, we performed a focused study that identifies the dimensions of ASD where customization has been considered on wearable and natural surfaces technologies, two of the most promising technologies for ASD, and assess the empirical evaluation that supports them. Our study revealed that, even though its critical importance, customization has fundamentally not been addressed in this domain and it opened avenues for research at the intersection of human-computer interaction and software engineering.

==> sections/future.tex <==
\section{Introduction}
\label{sec:introduction}

Here goes the text of the introduction ...

Here we start the paper ...This is the reference to the IT solutions book~\cite{Kientz2013} or another one~\cite{ANYAS/ElKalioubyPB06}.

Citing one from the primary sources~\citeS{S1-CHI/KientzA08}


